A Survey of Honeypots and Honeynets for Internet of Things, Industrial Internet of Things, and Cyber-Physical Systems

The Internet of Things (IoT), the Industrial Internet of Things (IIoT), and Cyber-Physical Systems (CPS) have become essential for our daily lives in contexts such as our homes, buildings, cities, health, transportation, manufacturing, infrastructure, and agriculture. However, they have become popular targets of attacks, due to their inherent limitations which create vulnerabilities. Honeypots and honeynets can prove essential to understand and defend against attacks on IoT, IIoT, and CPS environments by attracting attackers and deceiving them into thinking that they have gained access to the real systems. Honeypots and honeynets can complement other security solutions (i.e., firewalls, Intrusion Detection Systems - IDS) to form a strong defense against malicious entities. This paper provides a comprehensive survey of the research that has been carried out on honeypots and honeynets for IoT, IIoT, and CPS. It provides a taxonomy and extensive analysis of the existing honeypots and honeynets, states key design factors for the state-of-the-art honeypot/honeynet research and outlines open issues for future honeypots and honeynets for IoT, IIoT, and CPS environments.

==> Tables.tex <==
% Table generated by Excel2LaTeX from sheet '1st Table IoT'
  \begin{center}
  \twocolumn
  \LTcapwidth=\textwidth
  \begin{longtable}{|>{\footnotesize}p{2.5cm}|>{\footnotesize}c|>{\footnotesize}p{1.25cm}|>{\footnotesize}p{1.1cm}|>{\footnotesize}p{1.5cm}|>{\footnotesize}p{4.1cm}|>{\footnotesize}p{0.7cm}|>{\footnotesize}p{0.7cm}|>{\footnotesize}p{1.5cm}|}
  \caption{IoT Honeypots and Honeynets}\label{tab:iot-honeypots}\hline
    %\begin{tabular}{|p{11.59em}|c|p{5.455em}|p{3.955em}|p{5.365em}|p{23.59em}|p{3.18em}|p{3.32em}|p{4.365em}|}
    %\toprule
    \rowcolor[rgb]{ .141,  .251,  .384} \textcolor[rgb]{ 1,  1,  1}{\textbf{Work}} & {\textcolor[rgb]{ 1,  1,  1}{\textbf{Year}}} & \textcolor[rgb]{ 1,  1,  1}{\textbf{Level of Interaction}} & \textcolor[rgb]{ 1,  1,  1}{\textbf{Scalability}} & \textcolor[rgb]{ 1,  1,  1}{\textbf{Resource level}} & \textcolor[rgb]{ 1,  1,  1}{\textbf{Simulated services}} & \textcolor[rgb]{ 1,  1,  1}{\textbf{Role}} & \textcolor[rgb]{ 1,  1,  1}{\textbf{Open-source }} & \textcolor[rgb]{ 1,  1,  1}{\textbf{Application}} \\\endhead
   
    
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{HoneyD~\cite{HoneyD:2002}:2002}} & \cellcolor[rgb]{ 1,  1,  1}2002 & \cellcolor[rgb]{ 1,  1,  1}Low & \cellcolor[rgb]{ 1,  1,  1} \checkmark & \cellcolor[rgb]{ 1,  1,  1}Virtual (w/ physical  integration) & \cellcolor[rgb]{ 1,  1,  1}FTP, SMTP, Telnet,IIS, POP & \cellcolor[rgb]{ 1,  1,  1}Server & \cellcolor[rgb]{ 1,  1,  1}Yes & \cellcolor[rgb]{ 1,  1,  1}General \\\hline
    
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{Dionaea~\cite{Dionaea:2015}} & \cellcolor[rgb]{ 1,  1,  1}2009 & \cellcolor[rgb]{ 1,  1,  1}Medium & \cellcolor[rgb]{ 1,  1,  1}X & \cellcolor[rgb]{ 1,  1,  1}Virtual & \cellcolor[rgb]{ 1,  1,  1}Black hole, EPMAP, FTP, HTTP, Memache, Mirror, MongoDB, MQTT, MSSQL, MySQL, nfq, PPTP, SIP, SMB, TFTP, UPnP & \cellcolor[rgb]{ 1,  1,  1}Server & \cellcolor[rgb]{ 1,  1,  1}Yes & \cellcolor[rgb]{ 1,  1,  1} General \\\hline
    
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{Kippo~\cite{Kippo:2016}} & \cellcolor[rgb]{ 1,  1,  1}2009 & \cellcolor[rgb]{ 1,  1,  1}Medium & \cellcolor[rgb]{ 1,  1,  1} \checkmark & \cellcolor[rgb]{ 1,  1,  1}Virtual & \cellcolor[rgb]{ 1,  1,  1}SSH & \cellcolor[rgb]{ 1,  1,  1}Server & \cellcolor[rgb]{ 1,  1,  1}Yes & \cellcolor[rgb]{ 1,  1,  1}General \\\hline
    
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{Adaptive Honeypot Alternative (AHA) ~\cite{Wagener:2011}} & \cellcolor[rgb]{ 1,  1,  1}2011 & \cellcolor[rgb]{ 1,  1,  1}Low and High & \cellcolor[rgb]{ 1,  1,  1} \checkmark & \cellcolor[rgb]{ 1,  1,  1}Virtual & \cellcolor[rgb]{ 1,  1,  1}SSH & \cellcolor[rgb]{ 1,  1,  1}Server & \cellcolor[rgb]{ 1,  1,  1}Yes & \cellcolor[rgb]{ 1,  1,  1}General \\\hline
   
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{AHA with Rootkit Detection~\cite{Pauna:2012}} & \cellcolor[rgb]{ 1,  1,  1}2012 & \cellcolor[rgb]{ 1,  1,  1}Medium & \cellcolor[rgb]{ 1,  1,  1} \checkmark & \cellcolor[rgb]{ 1,  1,  1}Virtual & \cellcolor[rgb]{ 1,  1,  1}SSH & \cellcolor[rgb]{ 1,  1,  1}Server & \cellcolor[rgb]{ 1,  1,  1}No & \cellcolor[rgb]{ 1,  1,  1}General \\\hline
    
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{RASSH~\cite{Pauna:2014}} & \cellcolor[rgb]{ 1,  1,  1}2014 & \cellcolor[rgb]{ 1,  1,  1}Medium & \cellcolor[rgb]{ 1,  1,  1} \checkmark & \cellcolor[rgb]{ 1,  1,  1}Virtual & \cellcolor[rgb]{ 1,  1,  1}SSH & \cellcolor[rgb]{ 1,  1,  1}Server & \cellcolor[rgb]{ 1,  1,  1}Yes & \cellcolor[rgb]{ 1,  1,  1}General \\\hline
    
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{Cowrie~\cite{Cowrie:2019}} & \cellcolor[rgb]{ 1,  1,  1}2015 & \cellcolor[rgb]{ 1,  1,  1}Medium/High & \cellcolor[rgb]{ 1,  1,  1} \checkmark\newline{} & \cellcolor[rgb]{ 1,  1,  1}Virtual & \cellcolor[rgb]{ 1,  1,  1}SSH, Telnet, SFTP, SCP & \cellcolor[rgb]{ 1,  1,  1}Server & \cellcolor[rgb]{ 1,  1,  1}Yes & \cellcolor[rgb]{ 1,  1,  1}General \\\hline
    
     \rowcolor[rgb]{ .863,  .902,  .945} \textbf{HoneyPy~\cite{HoneyPy:2015}} & \cellcolor[rgb]{ 1,  1,  1}2015 & \cellcolor[rgb]{ 1,  1,  1}Low/Medium & \cellcolor[rgb]{ 1,  1,  1} \checkmark & \cellcolor[rgb]{ 1,  1,  1}Virtual & \cellcolor[rgb]{ 1,  1,  1}Created as required & \cellcolor[rgb]{ 1,  1,  1}Server & \cellcolor[rgb]{ 1,  1,  1}Yes & \cellcolor[rgb]{ 1,  1,  1}General \\\hline
     
     \rowcolor[rgb]{ .863,  .902,  .945} \textbf{IoTPOT (2015)~\cite{Pa:2015}} & \cellcolor[rgb]{ 1,  1,  1}2015 & \cellcolor[rgb]{ 1,  1,  1}Front end- Low Back end- High & \cellcolor[rgb]{ 1,  1,  1} \checkmark & \cellcolor[rgb]{ 1,  1,  1}Virtual & \cellcolor[rgb]{ 1,  1,  1}Telnet & \cellcolor[rgb]{ 1,  1,  1}Server & \cellcolor[rgb]{ 1,  1,  1}No & \cellcolor[rgb]{ 1,  1,  1}IoT \\\hline
    
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{Firmadyne~\cite{Chen:2016}} & \cellcolor[rgb]{ 1,  1,  1}2016 & \multicolumn{1}{l|}{\cellcolor[rgb]{ 1,  1,  1}High} & \multicolumn{1}{l|}{\cellcolor[rgb]{ 1,  1,  1} \checkmark} & \multicolumn{1}{l|}{\cellcolor[rgb]{ 1,  1,  1}Virtual} & \cellcolor[rgb]{ 1,  1,  1}Simulates full devices & \multicolumn{1}{l|}{\cellcolor[rgb]{ 1,  1,  1}Server} & \multicolumn{1}{l|}{\cellcolor[rgb]{ 1,  1,  1}Yes} & \cellcolor[rgb]{ 1,  1,  1}IoT \\\hline
  
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{IoT CandyJar~\cite{Luo:2017}} & \cellcolor[rgb]{ 1,  1,  1}2017 & \cellcolor[rgb]{ 1,  1,  1}Intelligent & \cellcolor[rgb]{ 1,  1,  1} \checkmark & \cellcolor[rgb]{ 1,  1,  1}Virtual & \cellcolor[rgb]{ 1,  1,  1}Simulates full devices  & \cellcolor[rgb]{ 1,  1,  1}Server & \cellcolor[rgb]{ 1,  1,  1}Yes & \cellcolor[rgb]{ 1,  1,  1}IoT \\\hline
   
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{Krishnaprasad (2017) ~\cite{Krishnaprasad:2017}} & \cellcolor[rgb]{ 1,  1,  1}2017 & \cellcolor[rgb]{ 1,  1,  1}High & \cellcolor[rgb]{ 1,  1,  1} \checkmark & \cellcolor[rgb]{ 1,  1,  1}Virtual\newline{} & \cellcolor[rgb]{ 1,  1,  1}Telnet, SSH, HTTP, CWMP & \cellcolor[rgb]{ 1,  1,  1}Server & \cellcolor[rgb]{ 1,  1,  1}Yes & \cellcolor[rgb]{ 1,  1,  1}IoT \\\hline
    
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{Anirudh et al.~\cite{Anirudh:2017}} & \cellcolor[rgb]{ 1,  1,  1}2017 & \cellcolor[rgb]{ 1,  1,  1}Low & \cellcolor[rgb]{ 1,  1,  1} \checkmark & \cellcolor[rgb]{ 1,  1,  1}Virtual & \cellcolor[rgb]{ 1,  1,  1}Not identified & \cellcolor[rgb]{ 1,  1,  1}Server & \cellcolor[rgb]{ 1,  1,  1}No & \cellcolor[rgb]{ 1,  1,  1}IoT \\\hline
   
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{HoneyIo4 Production Honeypot~\cite{Manzanares:2017}} & \cellcolor[rgb]{ 1,  1,  1}2017 & \cellcolor[rgb]{ 1,  1,  1}Low & \cellcolor[rgb]{ 1,  1,  1}X & \cellcolor[rgb]{ 1,  1,  1}Virtual & \cellcolor[rgb]{ 1,  1,  1}SNMP, SSH, SMTP, DNS, HTTP & \cellcolor[rgb]{ 1,  1,  1}Server & \cellcolor[rgb]{ 1,  1,  1}No & \cellcolor[rgb]{ 1,  1,  1}IoT \\\hline
   
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{Siphon~\cite{Guarnizo:2017}} & \cellcolor[rgb]{ 1,  1,  1}2017 & \cellcolor[rgb]{ 1,  1,  1}High & \cellcolor[rgb]{ 1,  1,  1} \checkmark & \cellcolor[rgb]{ 1,  1,  1}Physical & \cellcolor[rgb]{ 1,  1,  1}HTTP, Telnet, SSH, RTSP & \cellcolor[rgb]{ 1,  1,  1}Server & \cellcolor[rgb]{ 1,  1,  1}No & \cellcolor[rgb]{ 1,  1,  1}IoT \\\hline
    
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{MTPot~\cite{Evron:2017}} & \cellcolor[rgb]{ 1,  1,  1}2017 & \cellcolor[rgb]{ 1,  1,  1}Low & \cellcolor[rgb]{ 1,  1,  1}X & \cellcolor[rgb]{ 1,  1,  1}Virtual & \cellcolor[rgb]{ 1,  1,  1}Telnet & \cellcolor[rgb]{ 1,  1,  1}Server & \cellcolor[rgb]{ 1,  1,  1}Yes & \cellcolor[rgb]{ 1,  1,  1}IoT \\\hline
    
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{Semic and Mrdovic\cite{Semic:2017}} & \cellcolor[rgb]{ 1,  1,  1}2017 & \cellcolor[rgb]{ 1,  1,  1}Low & \cellcolor[rgb]{ 1,  1,  1} \checkmark & \cellcolor[rgb]{ 1,  1,  1}Virtual & \cellcolor[rgb]{ 1,  1,  1}Telnet & \cellcolor[rgb]{ 1,  1,  1}Server & \cellcolor[rgb]{ 1,  1,  1}No & \cellcolor[rgb]{ 1,  1,  1}IoT \\\hline
    
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{Pot2DPI~\cite{Martin:2017}} & \cellcolor[rgb]{ 1,  1,  1}2017 & \multicolumn{1}{l|}{\cellcolor[rgb]{ 1,  1,  1}Medium} & \multicolumn{1}{l|}{\cellcolor[rgb]{ 1,  1,  1} \checkmark} & \multicolumn{1}{l|}{\cellcolor[rgb]{ 1,  1,  1}Virtual} & \multicolumn{1}{l|}{\cellcolor[rgb]{ 1,  1,  1}Telnet, Upnp} & \multicolumn{1}{l|}{\cellcolor[rgb]{ 1,  1,  1}Server} & \multicolumn{1}{l|}{\cellcolor[rgb]{ 1,  1,  1}No} & \cellcolor[rgb]{ 1,  1,  1}Smart Home \\\hline
    
     \rowcolor[rgb]{ .863,  .902,  .945} \textbf{Metongnon et al.~\cite{Metongnon:2018}} & \cellcolor[rgb]{ 1,  1,  1}2018 & \cellcolor[rgb]{ 1,  1,  1}Low/Medium & \cellcolor[rgb]{ 1,  1,  1} \checkmark & \cellcolor[rgb]{ 1,  1,  1}Virtual & \cellcolor[rgb]{ 1,  1,  1}SSH, Telnet, EPMAP, FTP, HTTP, Memcache, MQTT, MSSQL, MySQL, PPTP, SIP, SMB, UPnP, TFTP, TR-069.1,TR-069.2, CoAP & \cellcolor[rgb]{ 1,  1,  1}Server & \cellcolor[rgb]{ 1,  1,  1}No & \cellcolor[rgb]{ 1,  1,  1}IoT \\\hline
    
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{QRASSH~\cite{Pauna:2018}} & \cellcolor[rgb]{ 1,  1,  1}2018 & \cellcolor[rgb]{ 1,  1,  1}Medium & \cellcolor[rgb]{ 1,  1,  1} \checkmark & \cellcolor[rgb]{ 1,  1,  1}Virtual & \cellcolor[rgb]{ 1,  1,  1}SSH & \cellcolor[rgb]{ 1,  1,  1}Server & \cellcolor[rgb]{ 1,  1,  1}Yes & \cellcolor[rgb]{ 1,  1,  1}General \\\hline
    
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{ThingPot et al.~\cite{Wang:2018}} & \cellcolor[rgb]{ 1,  1,  1}2018 & \cellcolor[rgb]{ 1,  1,  1}Medium & \cellcolor[rgb]{ 1,  1,  1} \checkmark & \cellcolor[rgb]{ 1,  1,  1}Virtual & \cellcolor[rgb]{ 1,  1,  1}HTTP, XMPP, ZigBee, & \cellcolor[rgb]{ 1,  1,  1}Server & \cellcolor[rgb]{ 1,  1,  1}Yes & \cellcolor[rgb]{ 1,  1,  1}Smart Home \\\hline
    
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{HIoTPOT~\cite{Gandhi:2018}} & \cellcolor[rgb]{ 1,  1,  1}2018 & \cellcolor[rgb]{ 1,  1,  1}High & \cellcolor[rgb]{ 1,  1,  1} \checkmark & \cellcolor[rgb]{ 1,  1,  1}Virtual & \cellcolor[rgb]{ 1,  1,  1}Not identified & \cellcolor[rgb]{ 1,  1,  1}Server & \cellcolor[rgb]{ 1,  1,  1}No & \cellcolor[rgb]{ 1,  1,  1}IoT \\\hline

    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{Stafira~\cite{Stafira:2019}} & \cellcolor[rgb]{ 1,  1,  1}2019 & \cellcolor[rgb]{ 1,  1,  1}Low & \cellcolor[rgb]{ 1,  1,  1} \checkmark & \cellcolor[rgb]{ 1,  1,  1}Physical & \cellcolor[rgb]{ 1,  1,  1}TCP/ IP, HTTP & \cellcolor[rgb]{ 1,  1,  1}Server & \cellcolor[rgb]{ 1,  1,  1}Yes & \cellcolor[rgb]{ 1,  1,  1}Smart Home \\\hline
   
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{IRASSH-T~\cite{Pauna:2019}} & \cellcolor[rgb]{ 1,  1,  1}2019 & \cellcolor[rgb]{ 1,  1,  1}Medium & \cellcolor[rgb]{ 1,  1,  1} \checkmark & \cellcolor[rgb]{ 1,  1,  1}Virtual & \cellcolor[rgb]{ 1,  1,  1}SSH & \cellcolor[rgb]{ 1,  1,  1}Server & \cellcolor[rgb]{ 1,  1,  1}Yes & \cellcolor[rgb]{ 1,  1,  1}IoT \\\hline
    
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{ML enhanced Cowrie~\cite{Shrivastava:2019}} & \cellcolor[rgb]{ 1,  1,  1}2019 & \cellcolor[rgb]{ 1,  1,  1}Medium & \cellcolor[rgb]{ 1,  1,  1} \checkmark & \cellcolor[rgb]{ 1,  1,  1}Virtual & \cellcolor[rgb]{ 1,  1,  1}SSH, Telnet & \cellcolor[rgb]{ 1,  1,  1}Server & \cellcolor[rgb]{ 1,  1,  1}Yes & \cellcolor[rgb]{ 1,  1,  1}IoT \\\hline
    
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{ML enhanced ThingPot~\cite{Vishwakarma:2019}} & \cellcolor[rgb]{ 1,  1,  1}2019 & \cellcolor[rgb]{ 1,  1,  1}Medium & \cellcolor[rgb]{ 1,  1,  1} \checkmark & \cellcolor[rgb]{ 1,  1,  1}Virtual & \cellcolor[rgb]{ 1,  1,  1}Telnet, MQTT, XMPP, AMQP, CoAP, UPnP, HTTP, REST & \cellcolor[rgb]{ 1,  1,  1}Server & \cellcolor[rgb]{ 1,  1,  1}No & \cellcolor[rgb]{ 1,  1,  1}IoT \\\hline
    
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{Scalable VPN- forwarded Honeypots~\cite{Tambe:2019}} & \cellcolor[rgb]{ 1,  1,  1}2019 & \cellcolor[rgb]{ 1,  1,  1}High & \cellcolor[rgb]{ 1,  1,  1} \checkmark & \cellcolor[rgb]{ 1,  1,  1}Physical & \cellcolor[rgb]{ 1,  1,  1}HTTP, TFTP, Telnet, others not specified & \cellcolor[rgb]{ 1,  1,  1}Server & \cellcolor[rgb]{ 1,  1,  1}No & \cellcolor[rgb]{ 1,  1,  1}IoT \\\hline
    
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{Zhang~\cite{Zhang:2019}} & \cellcolor[rgb]{ 1,  1,  1}2019 & \cellcolor[rgb]{ 1,  1,  1}Medium/High & \cellcolor[rgb]{ 1,  1,  1} \checkmark & \cellcolor[rgb]{ 1,  1,  1}Physical/ Virtual & \cellcolor[rgb]{ 1,  1,  1}UPnP, SOAP & \cellcolor[rgb]{ 1,  1,  1}Server & \cellcolor[rgb]{ 1,  1,  1}No & \cellcolor[rgb]{ 1,  1,  1}IoT \\\hline
    
     \rowcolor[rgb]{ .863,  .902,  .945} \textbf{U-Pot~\cite{HakimGithub:2019}} & \cellcolor[rgb]{ 1,  1,  1}2019 & \cellcolor[rgb]{ 1,  1,  1}Medium & \cellcolor[rgb]{ 1,  1,  1} \checkmark & \cellcolor[rgb]{ 1,  1,  1}Virtual & \cellcolor[rgb]{ 1,  1,  1}UPnP & \cellcolor[rgb]{ 1,  1,  1}Server & \cellcolor[rgb]{ 1,  1,  1}Yes & \cellcolor[rgb]{ 1,  1,  1}IoT \\\hline
    
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{HoneyCloud~\cite{Dang:2019}} & \cellcolor[rgb]{ 1,  1,  1}2019 & \cellcolor[rgb]{ 1,  1,  1}High & \cellcolor[rgb]{ 1,  1,  1} \checkmark & \cellcolor[rgb]{ 1,  1,  1}Physical/Virtual & \cellcolor[rgb]{ 1,  1,  1}SSH, Telnet, SMB, HTTP, HTTPS, RDP, MySQL, SQL Server & \cellcolor[rgb]{ 1,  1,  1}Server & \cellcolor[rgb]{ 1,  1,  1}No & \cellcolor[rgb]{ 1,  1,  1}Smart Home \\\hline
    
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{Phype~\cite{Phype:2019}} & \cellcolor[rgb]{ 1,  1,  1}2019 & \cellcolor[rgb]{ 1,  1,  1}Medium & \cellcolor[rgb]{ 1,  1,  1} \checkmark & \cellcolor[rgb]{ 1,  1,  1}Virtual & \cellcolor[rgb]{ 1,  1,  1}Telnet & \cellcolor[rgb]{ 1,  1,  1}Server & \cellcolor[rgb]{ 1,  1,  1}Yes\newline{} & \cellcolor[rgb]{ 1,  1,  1}IoT \\\hline
   
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{Chameleon~\cite{Zhou:2019}} & \cellcolor[rgb]{ 1,  1,  1}2019 & \multicolumn{1}{l|}{\cellcolor[rgb]{ 1,  1,  1}Medium} & \multicolumn{1}{l|}{\cellcolor[rgb]{ 1,  1,  1} \checkmark} & \cellcolor[rgb]{ 1,  1,  1}Physical/Virtual & \multicolumn{1}{l|}{\cellcolor[rgb]{ 1,  1,  1}Simulates full devices } & \multicolumn{1}{l|}{\cellcolor[rgb]{ 1,  1,  1}Server} & \multicolumn{1}{l|}{\cellcolor[rgb]{ 1,  1,  1}No} & \cellcolor[rgb]{ 1,  1,  1}IoT \\\hline
  
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{Honware~\cite{Vetterl:2019}} & \cellcolor[rgb]{ 1,  1,  1}2019 & \multicolumn{1}{l|}{\cellcolor[rgb]{ 1,  1,  1}High} & \multicolumn{1}{l|}{\cellcolor[rgb]{ 1,  1,  1} \checkmark} & \multicolumn{1}{l|}{\cellcolor[rgb]{ 1,  1,  1}Virtual} & \cellcolor[rgb]{ 1,  1,  1}Simulates full devices  & \multicolumn{1}{l|}{\cellcolor[rgb]{ 1,  1,  1}Server} & \multicolumn{1}{l|}{\cellcolor[rgb]{ 1,  1,  1}No} & \cellcolor[rgb]{ 1,  1,  1}IoT \\\hline
        
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{Lingenfelter et al.~\cite{Lingenfelter:2020}} & \cellcolor[rgb]{ 1,  1,  1}2020 & \multicolumn{1}{l|}{\cellcolor[rgb]{ 1,  1,  1}Medium} & \multicolumn{1}{l|}{\cellcolor[rgb]{ 1,  1,  1} \checkmark} & \multicolumn{1}{l|}{\cellcolor[rgb]{ 1,  1,  1}Virtual} & \cellcolor[rgb]{ 1,  1,  1}SSH, Telnet, SMTP, HTTP & \multicolumn{1}{l|}{\cellcolor[rgb]{ 1,  1,  1}Server} & \multicolumn{1}{l|}{\cellcolor[rgb]{ 1,  1,  1}Yes} & \cellcolor[rgb]{ 1,  1,  1}IoT \\\hline
    
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{Molina et al.~\cite{Molina:2020}} & \cellcolor[rgb]{ 1,  1,  1}2020 & \multicolumn{1}{l|}{\cellcolor[rgb]{ 1,  1,  1}High} & \multicolumn{1}{l|}{\cellcolor[rgb]{ 1,  1,  1} \checkmark} & \multicolumn{1}{l|}{\cellcolor[rgb]{ 1,  1,  1}Virtual} & \cellcolor[rgb]{ 1,  1,  1}Not identified & \multicolumn{1}{l|}{\cellcolor[rgb]{ 1,  1,  1}Server} & \multicolumn{1}{l|}{\cellcolor[rgb]{ 1,  1,  1}No} & \cellcolor[rgb]{ 1,  1,  1}IoT \\\hline
    


    
    %\end{tabular}%
  %
\end{longtable}%
\twocolumn
\end{center}



% Table generated by Excel2LaTeX from sheet '2ND TABLE'
\begin{table*}[htbp]
  \twocolumn
  %\centering
  \caption{IoT - Tool/Implementation/Attack Type}
    \begin{tabular}{|p{12.5em}|p{9.775em}|p{17.545em}|p{11em}|p{13.545em}|p{5.09em}|}
    \toprule
    \rowcolor[rgb]{ .141,  .251,  .384} \multicolumn{1}{|c|}{\textcolor[rgb]{ 1,  1,  1}{\textbf{Work}}} & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  1,  1}{\textbf{Tools}}} & \textcolor[rgb]{ 1,  1,  1}{\textbf{Simulated services}} & \textcolor[rgb]{ 1,  1,  1}{\textbf{Attack Type\newline{}}} & \textcolor[rgb]{ 1,  1,  1}{\textbf{Data analyzed}} & \textcolor[rgb]{ 1,  1,  1}{\textbf{Length of Study}} \\
    \midrule
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{HoneyD \cite{HoneyD:2002}:2002}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1} N/A} & \cellcolor[rgb]{ 1,  1,  1} FTP, SMTP, Telnet,IIS, POP & \cellcolor[rgb]{ 1,  1,  1} N/A & \cellcolor[rgb]{ 1,  1,  1} N/A & \cellcolor[rgb]{ 1,  1,  1} N/A \\
    \midrule
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{Dionaea \cite{Dionaea:2015}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1} N/A} & \cellcolor[rgb]{ 1,  1,  1} Black hole, EPMAP, FTP, HTTP, Memache, Mirror, MongoDB, MQTT, MSSQL, MySQL, nfq, PPTP, SIP, SMB, TFTP, UPnP & \cellcolor[rgb]{ 1,  1,  1} N/A & \cellcolor[rgb]{ 1,  1,  1} N/A & \cellcolor[rgb]{ 1,  1,  1} N/A \\
    \midrule
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{Kippo \cite{Kippo:2016}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1} N/A} & \cellcolor[rgb]{ 1,  1,  1} SSH & \cellcolor[rgb]{ 1,  1,  1} N/A & \cellcolor[rgb]{ 1,  1,  1} N/A & \cellcolor[rgb]{ 1,  1,  1} N/A \\
    \midrule
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{Adaptive Honeypot Alternative (AHA) \cite{Wagener:2011}} & \cellcolor[rgb]{ 1,  1,  1} AHA Daemon,  & \cellcolor[rgb]{ 1,  1,  1} SSH & \cellcolor[rgb]{ 1,  1,  1} SSH-brute force & \cellcolor[rgb]{ 1,  1,  1} user/passwords, TTY buffer, TCP/UDP packets & \cellcolor[rgb]{ 1,  1,  1} 8 hours \\
    \midrule
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{AHA with Rootkit Detection \cite{Pauna:2012}} & \cellcolor[rgb]{ 1,  1,  1} AHA Daemon,kernel rootkit Kbeast, Argos. & \cellcolor[rgb]{ 1,  1,  1} SSH & \cellcolor[rgb]{ 1,  1,  1} rootkit malware & \cellcolor[rgb]{ 1,  1,  1} keystroke logging, rootkit malware & \cellcolor[rgb]{ 1,  1,  1} 7 days \\
    \midrule
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{RASSH \cite{Pauna:2014}} & \cellcolor[rgb]{ 1,  1,  1} Pybrain RL, SARSA, Markov & \cellcolor[rgb]{ 1,  1,  1} SSH & \cellcolor[rgb]{ 1,  1,  1} SSH attack & \cellcolor[rgb]{ 1,  1,  1} logs, commands offering downloading & \cellcolor[rgb]{ 1,  1,  1} Not identified\newline{} \\
    \midrule
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{Cowrie \cite{Cowrie:2019}} & \cellcolor[rgb]{ 1,  1,  1} N/A & \cellcolor[rgb]{ 1,  1,  1} SSH, Telnet, SFTP, SCP & \cellcolor[rgb]{ 1,  1,  1} N/A & \cellcolor[rgb]{ 1,  1,  1} N/A & \cellcolor[rgb]{ 1,  1,  1} N/A \\
    \midrule
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{HoneyPy \cite{HONEYPY:2015}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1} N/A} & \cellcolor[rgb]{ 1,  1,  1} created as required & \cellcolor[rgb]{ 1,  1,  1} N/A & \cellcolor[rgb]{ 1,  1,  1} N/A & \cellcolor[rgb]{ 1,  1,  1} N/A \\
    \midrule
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{IoTPOT (2015) \cite{Pa:2015}} & \cellcolor[rgb]{ 1,  1,  1} masscan, pcap,  & \cellcolor[rgb]{ 1,  1,  1} Telnet & \cellcolor[rgb]{ 1,  1,  1} DNS Water Torture, SSL attack, DoS, DDoS, UDP Flood, SYN Flood, ACk Flood, SynAck Flood, Null Flood, Telnet Scan, DNS Attacks, Fake Web Hosting\newline{} & \cellcolor[rgb]{ 1,  1,  1} PCAP analysis includes total \# of packets, start/end time of packet captures, data\newline{}byte/bit rate, average packet size and rate, number of victim IP address for each attack & \cellcolor[rgb]{ 1,  1,  1} 39 days \\
    \midrule
    \rowcolor[rgb]{ .863,  .902,  .945} \multicolumn{1}{|c|}{\textbf{Firmadyne \cite{Chen:2016}}} & \cellcolor[rgb]{ 1,  1,  1} nmap, metasploit framework, binwalk, Scrapy, QEMU, sasquatch, firmware-mod-kit & \cellcolor[rgb]{ 1,  1,  1} HTTP, TELNET, DNS, dec-notes, HTTPS, UPnP, RIPD, freeciv & \cellcolor[rgb]{ 1,  1,  1} reconnaissance\newline{}attacks, buffer overflow & \cellcolor[rgb]{ 1,  1,  1} firmwares, results from web analysis, MIB files & \cellcolor[rgb]{ 1,  1,  1} not identified\newline{} \\
    \midrule
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{IoT CandyJar \cite{Luo:2017}} & \cellcolor[rgb]{ 1,  1,  1} pyLDAvis, Digital Ocean VM, Amazon AWS, MDP, Censys , ZoomEye, Shodan, MASSCAN & \cellcolor[rgb]{ 1,  1,  1} HTTP, RTSP, SOAP\_Envelope & \cellcolor[rgb]{ 1,  1,  1} HTTP, HTTP\_HEAD, udp, HTTP\_OPTIONS, tcp, RTSP, SOAP\_Envelope, HTTP\_CONNECT & \cellcolor[rgb]{ 1,  1,  1} Attack types and characteristics & \cellcolor[rgb]{ 1,  1,  1} 1 month \\
    \midrule
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{Krishnaprasad \cite{Krishnaprasad:2017}} & \cellcolor[rgb]{ 1,  1,  1} Twisted, ELK stack,Docker,  & \cellcolor[rgb]{ 1,  1,  1} Telnet, SSH, HTTP, CWMP & \cellcolor[rgb]{ 1,  1,  1} Bruteforce attack, hajime, ZmEu attacks & \cellcolor[rgb]{ 1,  1,  1} Attack types and characteristics & \cellcolor[rgb]{ 1,  1,  1} 7 days \\
    \midrule
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{Anirudh et al. \cite{Anirudh:2017}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1} IDS, logs} & \cellcolor[rgb]{ 1,  1,  1} Not identified & \cellcolor[rgb]{ 1,  1,  1} DoS Attacks & \cellcolor[rgb]{ 1,  1,  1} IP Address, MAC Address & \cellcolor[rgb]{ 1,  1,  1} not identified\newline{} \\
    \midrule
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{HoneyIo4 Production Honeypot \cite{Manzanares:2017}} & \cellcolor[rgb]{ 1,  1,  1} Shodan, Nmap, Wireshark, Scapy, VM. & \cellcolor[rgb]{ 1,  1,  1} SNMP, SSH, SMTP, DNS, HTTP & \cellcolor[rgb]{ 1,  1,  1} reconnaissance\newline{}attacks & \cellcolor[rgb]{ 1,  1,  1}  TCP, UDP and ICMP packets,  & \cellcolor[rgb]{ 1,  1,  1} not identfied\newline{} \\
    \midrule
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{Siphon \cite{Guarnizo:2017}} & \cellcolor[rgb]{ 1,  1,  1} Shodan, tcpdump, Nmap & \cellcolor[rgb]{ 1,  1,  1} HTTP, Telnet, SSH, RTSP & \cellcolor[rgb]{ 1,  1,  1} brute-force\newline{}login attempts & \cellcolor[rgb]{ 1,  1,  1} TCP connections per wormhole, services consulted, access gained, movements statistics  & \cellcolor[rgb]{ 1,  1,  1} 60 days \\
    \midrule
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{MTPot \cite{Evron:2017}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1} N/A} & \cellcolor[rgb]{ 1,  1,  1} Telnet & \cellcolor[rgb]{ 1,  1,  1} N/A & \cellcolor[rgb]{ 1,  1,  1}  incoming connections on any port using telnet & \cellcolor[rgb]{ 1,  1,  1} N/A \\
    \midrule
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{Semic and Mrdovic  \cite{Semic:2017}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1} N/A} & \cellcolor[rgb]{ 1,  1,  1} Telnet & \cellcolor[rgb]{ 1,  1,  1} telnet attack & \cellcolor[rgb]{ 1,  1,  1} protocols, IP addresses, logs & \cellcolor[rgb]{ 1,  1,  1} not identified\newline{} \\
    \midrule
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{Pot2DPI \cite{Martin:2017}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1} N/A} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1} telnet, upnp} & \cellcolor[rgb]{ 1,  1,  1} mirai and Persirai attacks protocols, ports scans  & \cellcolor[rgb]{ 1,  1,  1} packet traces, attack signatures, protocols, ports, & \cellcolor[rgb]{ 1,  1,  1} not identified\newline{} \\
    \midrule
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{Metongnon et al. \cite{Metongnon:2018}} & \cellcolor[rgb]{ 1,  1,  1} eemo,  Shodan  & \cellcolor[rgb]{ 1,  1,  1} SSH, Telnet, EPMAP, FTP, HTTP, Memcache, MQTT, MSSQL, MySQL, PPTP, SIP, SMB, UPnP, TFTP, TR-069.1,TR-069.2, CoAP & \cellcolor[rgb]{ 1,  1,  1} attack URL, SYN packet, Mirai and Mirai-like attacks, harvest\newline{}crypto-currencies, login attempts, reconaissance & \cellcolor[rgb]{ 1,  1,  1} Protocols, packets per port, packets characteristics & \cellcolor[rgb]{ 1,  1,  1} 5 months \\
    \midrule
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{QRASSH \cite{Pauna:2018}} & \cellcolor[rgb]{ 1,  1,  1} Deep Q-learning, Keras with Theano backend, nmap & \cellcolor[rgb]{ 1,  1,  1} SSH & \cellcolor[rgb]{ 1,  1,  1} SSH attack & \cellcolor[rgb]{ 1,  1,  1} commands( downloading,hacking, linux) & \cellcolor[rgb]{ 1,  1,  1} Not identified\newline{} \\
    \midrule
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{ThingPot et al. \cite{Wang:2018}} & \cellcolor[rgb]{ 1,  1,  1} skipfish, nikto, masscan & \cellcolor[rgb]{ 1,  1,  1} HTTP, XMPP, ZigBee, & \cellcolor[rgb]{ 1,  1,  1} HTTP POST request,HTTP GET with URLs,scanning tools, SQL malware, & \cellcolor[rgb]{ 1,  1,  1} HTTP request, SQL access request, scanning network & \cellcolor[rgb]{ 1,  1,  1} 1.5 months \\
    \midrule
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{Stafira \cite{Stafira:2019}} & \cellcolor[rgb]{ 1,  1,  1} nmap, wireshark, VMWareWorkstation  & \cellcolor[rgb]{ 1,  1,  1} TCP/ IP, HTTP & \cellcolor[rgb]{ 1,  1,  1} only user testing & \cellcolor[rgb]{ 1,  1,  1} access time, HTML code, network headers,\newline{}and Nmap scan & \cellcolor[rgb]{ 1,  1,  1} Not identified\newline{} \\
    \midrule
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{IRASSH-T \cite{Pauna:2019}} & \cellcolor[rgb]{ 1,  1,  1} Apprenticeship Learning & \cellcolor[rgb]{ 1,  1,  1} SSH & \cellcolor[rgb]{ 1,  1,  1} SSH attack & \cellcolor[rgb]{ 1,  1,  1} N/A & \cellcolor[rgb]{ 1,  1,  1} N/A \\
    \midrule
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{ML enhanced Cowrie \cite{Shrivastava:2019}} & \cellcolor[rgb]{ 1,  1,  1} Support Vector Machine (SVM), Random Forest, Naive Bayes, J48 decision tree, virustotal website, Weka, machine learning algorithms & \cellcolor[rgb]{ 1,  1,  1} SSH, Telnet & \cellcolor[rgb]{ 1,  1,  1} malicious payload, SSH attack, XOR DDoS, Spying, Suspicious, Clean & \cellcolor[rgb]{ 1,  1,  1} System logs, IP, attack types and characteristics, commands executed, behavior analysis & \cellcolor[rgb]{ 1,  1,  1} 40 days \\
    \midrule
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{ML enhanced ThingPot \cite{Vishwakarma:2019}} & \cellcolor[rgb]{ 1,  1,  1} Linux bash scripts, Microsoft\newline{}Azure, MATLAB & \cellcolor[rgb]{ 1,  1,  1} Telnet, MQTT, XMPP, AMQP, CoAP, UPnP, HTTP, REST & \cellcolor[rgb]{ 1,  1,  1} DDoS, malware, TCP\newline{}SYN flood, UDP flood,HTTP GET flood & \cellcolor[rgb]{ 1,  1,  1} network traffic, payload, malware samples, the toolkit by attacker & \cellcolor[rgb]{ 1,  1,  1} Not identified\newline{} \\
    \midrule
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{Scalable VPN- forwarded Honeypots \cite{Tambe:2019}} & \cellcolor[rgb]{ 1,  1,  1} VPN,TShark, HONAN, pcap, VM, MySQL, own script & \cellcolor[rgb]{ 1,  1,  1} HTTP, TFTP, Telnet, others not specified & \cellcolor[rgb]{ 1,  1,  1} DDoS style attacks & \cellcolor[rgb]{ 1,  1,  1} Protocols, packets per port, packets characteristics & \cellcolor[rgb]{ 1,  1,  1} 16 months \\
    \midrule
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{Zhang \cite{Zhang:2019}} & \cellcolor[rgb]{ 1,  1,  1} Tc, own script & \cellcolor[rgb]{ 1,  1,  1} UPnP, SOAP & \cellcolor[rgb]{ 1,  1,  1} UPnP & \cellcolor[rgb]{ 1,  1,  1} Protocols, packets per port,  timestamp, inject behaviors & \cellcolor[rgb]{ 1,  1,  1} 7 days \\
    \midrule
     \rowcolor[rgb]{ .863,  .902,  .945} \textbf{U-Pot \cite{HakimGithub:2019}} & \cellcolor[rgb]{ 1,  1,  1} shodan, Zmap, U- Pot & \cellcolor[rgb]{ 1,  1,  1} UPnP & \cellcolor[rgb]{ 1,  1,  1} N/A & \cellcolor[rgb]{ 1,  1,  1} N/A & \cellcolor[rgb]{ 1,  1,  1} N/A \\
    \midrule
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{HoneyCloud \cite{Dang:2019}} & \cellcolor[rgb]{ 1,  1,  1} VM. Cloud storage, antivirus communities, Honeycomb, virustotal website & \cellcolor[rgb]{ 1,  1,  1} SSH, Telnet, SMB, HTTP, HTTPS, RDP, MySQL, SQL Server & \cellcolor[rgb]{ 1,  1,  1} Fileless attacks, malware-based attacks,  & \cellcolor[rgb]{ 1,  1,  1} symmetry/asymmetry of data flows, packets analysis, attack types and characteristics, keystrokes, trace of network activities, CPU usage, Process list. & \cellcolor[rgb]{ 1,  1,  1} 1  year \\
    \midrule
     \rowcolor[rgb]{ .863,  .902,  .945} \textbf{Phype \cite{Phype:2019}} & \cellcolor[rgb]{ 1,  1,  1} Phype Telnet & \cellcolor[rgb]{ 1,  1,  1} Telnet & \cellcolor[rgb]{ 1,  1,  1} N/A & \cellcolor[rgb]{ 1,  1,  1} N/A & \cellcolor[rgb]{ 1,  1,  1} N/A \\
    \midrule
    \rowcolor[rgb]{ .863,  .902,  .945} \multicolumn{1}{|c|}{\textbf{Chamaleon \cite{Zhou:2019}}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1} nmap, shodan} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1} Not identified} & \cellcolor[rgb]{ 1,  1,  1} reconnaissance\newline{}attacks & \cellcolor[rgb]{ 1,  1,  1} IP whitelist, received requests & \cellcolor[rgb]{ 1,  1,  1} Not identified\newline{} \\
    \midrule
    \rowcolor[rgb]{ .863,  .902,  .945} \multicolumn{1}{|c|}{\textbf{Honware \cite{Vetterl:2019}}} & \cellcolor[rgb]{ 1,  1,  1} QEMU, binwalk, wireshark, ping, nmap, Firmadyne, Shodan  & \cellcolor[rgb]{ 1,  1,  1} SSH, telnet, HTTP, UPnP, DHCP, DNS, dec-notes, freciv, netbios, HTTPS, MDNS, TFTP & \cellcolor[rgb]{ 1,  1,  1} reconnaissance\newline{}attacks, Zero days, capture attacks traffic & \cellcolor[rgb]{ 1,  1,  1} kernel logs, firmwares, & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1} < 2 months} \\
    \midrule
    \rowcolor[rgb]{ .863,  .902,  .945} \textbf{Lingenfelter \cite{Lingenfelter:2020}} & \cellcolor[rgb]{ 1,  1,  1} Filebeat, ELK stack, Logstash, VirusTotal,  & \cellcolor[rgb]{ 1,  1,  1} SSH, Telnet & \cellcolor[rgb]{ 1,  1,  1} IoT botnet malware & \cellcolor[rgb]{ 1,  1,  1} Packets per port, System logs, IPs, Brute-force scan, file hash  & \cellcolor[rgb]{ 1,  1,  1} 40 days\newline{} \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table*}%




